Bayesian workflow for disease transmission modeling in Stan

This tutorial shows how to build, fit, and criticize disease transmission models in Stan, and should be useful to researchers interested in modeling the SARS-CoV-2 pandemic and other infectious diseases in a Bayesian framework. Bayesian modeling provides a principled way to quantify uncertainty and incorporate both data and prior knowledge into the model estimates. Stan is an expressive probabilistic programming language that abstracts the inference and allows users to focus on the modeling. As a result, Stan code is readable and easily extensible, which makes the modeler's work more transparent. Furthermore, Stan's main inference engine, Hamiltonian Monte Carlo sampling, is amiable to diagnostics, which means the user can verify whether the obtained inference is reliable. In this tutorial, we demonstrate how to formulate, fit, and diagnose a compartmental transmission model in Stan, first with a simple Susceptible-Infected-Recovered (SIR) model, then with a more elaborate transmission model used during the SARS-CoV-2 pandemic. We also cover advanced topics which can further help practitioners fit sophisticated models; notably, how to use simulations to probe the model and priors, and computational techniques to scale-up models based on ordinary differential equations.

==> simdata.tex <==
 


==> simplesir.tex <==

\subsection{Data}

In this example, we examine an outbreak of influenza A (H1N1) in 1978 at a British boarding school. 
The data consists of the daily number of students in bed, spanning over a time interval of 14 days from January 22nd to February 4th (figure 1A).
% make a figure with the raw data in the A panel
There were 763 male students who were mostly full boarders and 512 of them became ill.  
It is reported that one infected boy started the epidemic, which spread rapidly in the relatively closed community of the boarding school. 
The data are freely available in the \texttt{R} package \texttt{outbreaks}, maintained as part of the R Epidemics Consortium \footnote{\url{https://www.repidemicsconsortium.org/}}.

\subsection{Transmission model} 

The Susceptible-Infected-Recovered (SIR) model splits the population in three time-dependent compartments: the susceptible, infected (and infectious), and recovered (and not infectious) compartments. 
When a susceptible individual comes into contact with an infectious individual, the former can become infected for some time, and then recover and become immune. 
The dynamics can be summarized graphically (figure 1B), or by the following system of ODEs:
% put the diagram in the B panel of figure 1
\begin{align}
	\frac{dS}{dt} &= -\beta  S(t) \frac{I(t)}{N}\\
	\frac{dI}{dt} &= \beta  S(t)  \frac{I(t)}{N} - \gamma  I(t) \\
	\frac{dR}{dt} &= \gamma I(t),
\end{align}
where $S(t)$ is the number of people susceptible to becoming infected (no immunity),  $I(t)$ is the number of people currently infected (and infectious) and $R(t)$ is the number of recovered people (we assume they remain immune indefinitely).
In such a short time span we can consider the total population as stable with size $N=S(t)+I(t)+R(t)$.
Two parameters govern the dynamics of the system: $\beta$ is the rate of infectious contact between people and $\gamma$ the recovery rate of infected individuals.
Both parameters are assumed to be constant with time.

Let's give some intuition behind these equations. 
The proportion of infected people in the population at time $t$ is $\frac{I (t)}{N}$. 
At each time step, assuming homogeneous mixing, the probability for a susceptible person to become infected is thus $\beta\frac{I(t)}{N}$, with $\beta$ the average number of contacts per person per time multiplied by the probability of disease transmission when a susceptible and an infected subject come in contact. 
Hence, at each time step, $\beta  S(t) \frac{I(t)}{N}$ susceptible individuals become infected, thus leave the $S$ compartment to enter the $I$ compartment. 
Similarly, the recovery of an infected individual is taking place at rate $\gamma$, and therefore the number of infected individuals decreases with speed $\gamma I(t)$ while the number of recovered grows at the same speed.


The above model holds under several assumptions: 
\begin{itemize}[noitemsep,nolistsep]
\item  births and deaths are not contributing to the dynamics and the total population $N$ remains constant, 
\item  recovered individuals do not become susceptible again over the considered period,
\item  the infection rate $\beta$ and recovery rate $\gamma$ are constant, 
\item  the population is homogeneous, 
\item  individuals meet any other individual uniformly at random (homogeneous mixing) and recovery time follows an exponential distribution with mean $\frac{1}{\gamma}$,
\item  replacing the integer number of people in each compartment by a continuous approximation is acceptable.
\end{itemize}
In case of boarding school data, the spread of the disease has started with one infected individual which leads to the initial conditions $I(0) = 1, S(0) = N-1, R(0) = 0$.

\subsection{Statistical model} 

We now introduce a \textit{sampling distribution} (also termed likelihood)
$$ 
p(\mathcal Y \mid \theta) 
$$
which tells us, given model parameters $\theta$, how to generate data $\mathcal Y$.
Inference reverse-engineers the data generating process
and asks: "given a model and observations, $\mathcal Y$,
what are plausible parameter values?"
In a Bayesian framework, the set of plausible values is characterized by
the \textit{posterior distribution}, 
$$
p(\theta \mid \mathcal Y)
$$
Bayes' rule teaches us that
$$
p(\theta \mid \mathcal Y) \propto p(\mathcal Y \mid \theta) p(\theta)
$$
where $p(\mathcal Y \mid \theta)$ is the sampling distribution,
$p(\theta)$ the \textit{prior distribution},
and $\propto$ stands for "proportional to".
The prior encodes information about the parameter values that is available before observing the data.
To summarize, a Bayesian model couples a mathematical model of what we know about the parameters in the form of a prior and a sampling distribution, i.e. a model of the data generating process.

%<!-- ^[Given the a priori probability of the parameters $p(\theta)$ and the probability of the data given the parameters $p(y|\theta)$, Bayes rules tells us that the posterior distribution of the parameters $\theta$ is $p(\theta|y) \propto p(\theta)p(y|\theta)$]. Specifically, a Bayesian model requires a mathematical model of what we know about the parameters (i.e., a prior) and a model of what we know about the data generating process given the parameters (i.e., a sampling distribution). -->

\subsection{Sampling distribution}

Given parameter values and initial conditions, a compartmental model defines a unique solution for the sizes of the compartments in time, including the number of infected students, $I_\text{ODE}(t)$. 
We want to link this solution to the observed data, i.e the number of students in bed at each time point $I_\text{obs}(t)$.
The latter is a noisy estimate of the true number of infected students.
We choose to model the number of students in bed with a count distribution -- the negative binomial distribution. 
This distribution allows us to use $I_\text{ODE}(t)$ as the expected value and account for over-dispersion through an additional parameter $\phi$:

\begin{equation}
I_\text{obs}(t) \sim \text{NegBin}\left(I_\text{ODE}(t), \phi \right)
\end{equation}

This gives us $p(\mathcal Y \mid \theta)$, with $\theta = \{\beta, \gamma, \phi\}$ the three model parameters.
	
\subsection{Prior distribution}

We now need to specify $p(\theta)$. 
With $\theta = (\beta, \gamma, \phi)$, we select a prior distribution for each of the three parameters. 
One advantage of the Bayesian approach is that we can formally incorporate prior domain knowledge about the parameter values into the model.
For instance, we specify $\gamma \sim N(0.4, 0.5)$ (truncated at 0), which expresses our belief that $\gamma$ has to be positive, and that $P(\gamma \leq 1) = 0.9$ (i.e the probability that the recovery time is longer than a day is 0.9). 
We can change this prior if more information becomes available, constraining our parameter estimation more tightly or, on the contrary, increasing its variance.
Section \ref{sec:simdata} discusses how to check if the chosen priors are consistent with available domain knowledge using \textit{prior predictive checks}.

\subsection{Predictions and derived quantities}

Once we fit the model and obtain a posterior distribution for $\theta$, we can derive additional quantities of interests.
We can simulate predictions, $\mathcal Y_\mathrm{pred}$,
and work out the plausible range of new observations.
Because these predictions are based on the posterior, $p(\theta \mid \mathcal Y)$,
our simulations account for uncertainty both in the data generating process
and in our estimates of $\theta$.
Moreover, we compute the posterior distribution of predictions
\begin{equation}
p(\mathcal Y_\mathrm{pred} \mid \mathcal Y) = \int p(\mathcal Y_{pred} | \theta) p(\theta | \mathcal Y) d\theta
\end{equation}

Similarly we can compute quantities that depend on the model parameters.
An important example is the basic reproduction number, $R_0$.
$R_0$ is defined as the expected number of secondary infections produced from one infected individual in a fully susceptible population through the entire duration of the infectious period.
$R_0 > 1$ indicates a sustainable infection,
which can lead to a major outbreak, while $R_0 < 1$ suggests, under stable conditions, that the infection will die out.
Within the simple SIR model, this quantity is defined as
\begin{equation}
R_0 = \frac{\beta}{\gamma}
\end{equation}
Bayesian inference allows us to construct a posterior distribution for this quantity too
\begin{equation}
p(R_0 \mid \mathcal Y)
\end{equation}


\subsection{Coding the model in \texttt{Stan}}


We will need the following libraries:
\begin{verbatim}
library(rstan)
library(gridExtra)
rstan_options (auto_write = TRUE)
options (mc.cores = parallel::detectCores ())
set.seed(3) # for reproductibility
\end{verbatim}

\subsubsection{Coding the ODE in \texttt{Stan}}

An ODE takes the form
\begin{equation}
\frac{\mathrm d y}{\mathrm d t} = f(t, y)
\end{equation}
where $y$ are the states, in our example $y = (S, I, R)$, and $t$ is time.
We also need an initial condition $y_0$ at $t_0$ and the times  at which we evaluate the solution $\tau$.

To specify an ODE in Stan, we first code $f$ in the \texttt{functions} block.
This function must observe a strict signature:
\begin{verbatim}
real[] f(real time, real[] state, real[] theta, real[] x_r, int[] x_i)
\end{verbatim}
with
\begin{itemize}[noitemsep,nolistsep]
\item  \texttt{time}, $t$;
\item  \texttt{state}, the volumes in each compartment, $y$;
\item  \texttt{theta}, variables used to compute $f$, which depend on the model parameters;
\item  \texttt{x\_r}, real variables used to evaluate $f$, which only depend on fixed data;
\item  \texttt{x\_i}, integer values used to evaluate $f$, which only depend on fixed data.
\end{itemize}
We motivate this signature in our discussion on scaling ODEs (section \ref{sec:scaleup}).
In our example, the ODEs for the SIR model is defined as follows:
\begin{verbatim}
functions {
	real[] sir(real t, real[] y, real[] theta, 
	real[] x_r, int[] x_i) {
		
		real S = y[1];
		real I = y[2];
		real R = y[3];
		real N = x_i[1];
		
		real beta = theta[1];
		real gamma = theta[2];
		
		real dS_dt = -beta * I * S / N;
		real dI_dt =  beta * I * S / N - gamma * I;
		real dR_dt =  gamma * I;
		
		return {dS_dt, dI_dt, dR_dt};
	}
}
\end{verbatim}

We evaluate the solution numerically by using one of Stan's numerical integrators.
We opt for the Runge-Kutta 4$^\mathrm{th}$ / 5$^\mathrm{th}$ order
but, as we discuss in section \ref{sec:scaleup}, the user can consider other options.
A call to the integrator looks as follows
\begin{verbatim}
y = integrate_ode_rk45(sir, y0, t0, ts, theta, x_r, x_i);
\end{verbatim}
with
\begin{itemize}[noitemsep,nolistsep]
\item  \texttt{sir}, the name of the function that returns the derivatives, $f$;
\item  \texttt{y0}, the initial condition;
\item  \texttt{t\_0}, the time of the initial condition;
\item  \texttt{ts}, the times at which we require the solution to be evaluated;
\item  \texttt{theta}, \texttt{x\_r}, \texttt{x\_i}, arguments to be passed to $f$.
\end{itemize}
We now have all the ingredients to solve the system of ODEs.
Note that in the given example, when we assume that the total population remains constant, the three derivatives $\frac{dS}{dt}$, $\frac{dI}{dt}$, $\frac{dR}{dt}$ sum up to $0$.
 We can use this fact to improve computational efficiency of the \texttt{sir} function by deriving the value of $\frac{dI}{dt}$ from $\frac{dS}{dt}$ and $\frac{dR}{dt}$:
\begin{verbatim}
real dS_dt = -beta * I * S / N;
real dR_dt =  gamma * I;
real dI_dt =  -(dS_dt + dR_dt);
\end{verbatim}

\subsubsection{Building the model in \texttt{Stan}}

We next code the model in \texttt{Stan}, working through the various coding blocks.
The \texttt{`functions`} block specifies \texttt{`sir`}
\begin{verbatim}
functions {
	real[] sir (...) {...} //copy code from above
}
\end{verbatim}

Fixed data is declared in the \texttt{data} block:
\begin{verbatim}
data {
	int<lower=1> n_days;
	real y0[3];
	real t0;
	real ts[n_days];
	int N;
	int cases[n_days];
}
\end{verbatim}

We code transforms of the data in the \texttt{transformed data} block. 
In this example, we transform our data  to match the signature of \texttt{sir} (with \texttt{x\_r} being of length 0 because we have nothing to put in it).
\begin{verbatim}
transformed data {
	real x_r[0];
	int x_i[1] = { N };
}
\end{verbatim}

We next declare the model parameters. 
If you want some parameter to be bounded, and it is not already guaranteed by his prior, you need to specify \texttt{<lower=a, upper=b>} when declaring this parameter. Note that this is how you put a truncated prior distribution on a parameter.

\begin{verbatim}
parameters {
	real<lower=0> gamma;
	real<lower=0> beta;
	real<lower=0> phi_inv;
}
\end{verbatim}

And then transforms of the parameters
\begin{verbatim}
transformed parameters{
	real y[n_days, 3];
	real phi = 1. / phi_inv;
	{
		real theta[2];
		theta[1] = beta;
		theta[2] = gamma;
		
		y = integrate_ode_rk45(sir, y0, t0, ts, theta, x_r, x_i);
	}
}
\end{verbatim}


With the ODE solution, $y$, in hand, the only thing left to do is to code the prior and sampling distribution. 
%<!-- As with the other parts of the model, these directly follow the notation in the mathematical specification. -->
\begin{verbatim}
model {
	//priors
	beta ~ normal(2, 1); //truncated at 0
	gamma ~ normal(0.4, 0.5); //truncated at 0
	phi_inv ~ exponential(5);
	
	//sampling distribution
	//col(matrix x, int n) - The n-th column of matrix x. Here the number of infected people
	cases ~ neg_binomial_2(col(to_matrix(y), 2), phi);
}
\end{verbatim}


Untangled from the inference, we can calculate the basic reproduction number, $R_0$, and predictions for the number of cases in the \texttt{generated quantities} block:
\begin{verbatim}
generated quantities {
	real R0 = beta / gamma;
	real recovery_time = 1 / gamma;
	real pred_cases[n_days];
	pred_cases = neg_binomial_2_rng(col(to_matrix(y), 2) + 1e-5, phi);
}
\end{verbatim}


\subsubsection{Fitting the model in \texttt{R}}

%<!-- To provide the data to Stan for inference -->
%<!-- ^[What do we mean by inference here? We want to infer the value of the parameters $\theta$ given the data $y$ . We have already specified the priors $p(\theta)$ and the likelihood $p(y|\theta)$. Bayes rules tells us that the posterior distribution of the parameters $\theta$ is $p(\theta|y) \propto p(\theta)p(y|\theta)$. We thus know this distribution $p(\theta|y)$ up to a multiplicative constant. Stan provides a version of Markov Chain Monte Carlo (MCMC), which provides samples which approximativelly follow the $p(\theta|y)$ distribution. By approximating the true posterior distribution by the empirical distribution on these samples, we can compute the expectations of functions of the paramaters, or e.g the probability that the number of infected student is more than 10 on the third day.],  -->
%<!-- we collect it into a list -->
We now go to \texttt{R} and collect the data into a list.
\begin{verbatim}
# time series of cases
cases <- influenza_england_1978_school$in_bed  # Number of students in bed

# total count
N <- 763

# times
n_days <- length(cases) 
t <- seq(0, n_days, by = 1)
t0 = 0 
t <- t[-1]

# initial conditions
i0 <- 1
s0 <- N - i0
r0 <- 0
y0 = c(S = s0, I = i0, R = r0)

# data for Stan
data_sir <- list(n_days = n_days, y0 = y0, t0 = t0, ts = t, N = N, cases = cases)

# number of MCMC steps
niter <- 2000
\end{verbatim}

Next we compile the model, saved in the file \texttt{sir\_negbin.stan},
\begin{verbatim}
model <- stan_model("sir_negbin.stan")
\end{verbatim}
and run MCMC.
For this problem, it suffices to use Stan's defaults.
Note that, as is standard practice, we run 4 Markov chains.
\begin{verbatim}
fit_sir_negbin <- sampling(model, data = data_sir, iter = niter, chains = 4)
\end{verbatim}

\subsubsection{Checking the inference}

We first specify the parameters of interest.
\begin{verbatim}
pars=c('beta', 'gamma', "R0", "recovery_time")
\end{verbatim}
%<!-- We here display the median (0.5 quantile) and 90% interval (0.05 and 0.95 quantiles), restricted to the parameters of interest. -->
We start with a summary table of the results,
which displays the posterior mean, standard error, quantiles,
and some useful diagnostics.
\begin{verbatim}
print(fit_sir_negbin, pars = pars)
\end{verbatim}

\texttt{Stan} gives us a host of information to evaluate whether the inference is reliable. 
During sampling, warnings can tell us if something is wrong (here we have no warnings
\footnote{Note that getting a few warnings is not always concerning, especially if they only occur during
the warmup phase. See \url{https://mc-stan.org/misc/warnings.html} for an overview of Stan's warnings]}. 
In the summary table, several quantities are available to check inference. 
Here we note that $\widehat R$ is close to 1 (< 1.01),
indicating the 4 Markov chains are in close agreement with one another.
Furthermore the effective samples size, $n_\mathrm{eff}$, is large (> 100\footnote{$n_\mathrm{eff} \geq 100$ is considered sufficient to estimate the posterior mean correctly. Note that we may need a bigger $n_\mathrm{eff}$ to estimate extreme quantiles.}),
which means the Markov chains were able to cohesively explore the parameter space.
Conversely, large $\widehat R$ and low $n_\mathrm{eff}$ would indicate that the Markov chains
are poorly mixing. 
Apart from fixing coding errors, improving the mixing of the Markov chains almost always requires tweaking the model specification, for example with a reparameterization \footnote{\url{https://mc-stan.org/docs/2_23/stan-users-guide/reparameterization-section.html}} or stronger priors.

%<!-- There were no divergent transitions reported^[Divergences occur when Stan’s Hamiltonian solver diverges from the true Hamiltonian, which must be conserved, because of numerical problems in the stepwise gradient-based approximation of the curvature of the log density. This indicates that the Markov chains did not completely explore the posterior and that our Markov chain Monte Carlo estimators will be biased. This is often the sign that some region of the posterior is hard to explore and that the step-size strongly depends on the location. Divergences, however, can sometimes be false positives. To verify that we have real fitting issues we can rerun with a larger target acceptance probability, adapt_delta, which will force more accurate simulations of Hamiltonian trajectories and reduce the false positives.] and more generally no warning messages.  -->
%<!-- $\hat{R}$ values^[$\hat{R}$ indicates how well different chains of the MCMC have mixed : if $\hat{R}$ is close to 1, it means that all the chains are exploring the same region, and thus that no chain should be stuck in one subregion. In practice, $\hat{R} \leq 1.01$ is satisfactory.] are close to 1 (<1.01), and the effective sample size^[The effective sample size corresponds to the number of independant posterior draws which would yield the same standard error of estimation for the **mean** of the parameters that the draws from Stan's MCMC. Note that $n_{eff}$ can be much lower for quantiles. In practice, $n_{eff} \geq 100$ for estimating the parameter mean is considered sufficient. With effective sample sizes of roughly one hundred, standard errors are roughly one tenth the size of posterior standard deviations, being in an inverse square root relation.] estimates for each parameter are sufficient (>100) for inference^[Both large $\hat{R}$ and low effective samples per transition would be consequences of poorly mixing Markov chains. Improving the mixing of the Markov chains almost always requires tweaking the model specification, for example with a reparameterization or stronger priors.]. -->

We can furthermore plot the marginal posterior densities
and confirm the Markov chains are in agreement with one another.
\begin{verbatim}
stan_dens(fit_sir_negbin, pars = pars, separate_chains = TRUE)
\end{verbatim}


\subsubsection{Checking the model}

Now that we trust our inference, let us check the utility of our model.
Utility is problem specific and can include the
precise estimation of a quantity or predicting future behaviors.
In general, it is good to check if our model, once fitted, produces simulations
that are consistent with the observed data.
This is the idea behind \textit{posterior predictive checks}.

We sample predictions, $\mathcal Y_\mathrm{pred}$, 
from $p(\mathcal Y_\mathrm{pred} \mid \mathcal Y)$
and use these samples to construct a fitted curve for students in bed,
together with the uncertainty (90% interval, 
meaning observed data is expected to fall outside of this interval one in ten times). 
This posterior predictive check allows us to verify if the model captures the structure of the data. 
Here we see that the model gives a satisfying fit to the data, 
and that the model uncertainty is able to capture the variation of the data.

\begin{verbatim}
smr_pred <- cbind(as.data.frame(summary(
fit_sir_negbin, pars = "pred_cases", probs = c(0.05, 0.5, 0.95))$summary), t, cases)
colnames(smr_pred) <- make.names(colnames(smr_pred)) # to remove % in the col names

ggplot(smr_pred, mapping = aes(x = t)) +
geom_ribbon(aes(ymin = X5., ymax = X95.), fill = "orange", alpha = 0.6) +
geom_line(mapping = aes(x = t, y = X50.)) + 
geom_point(mapping = aes(y = cases)) +
labs(x = "Day", y = "Number of students in bed")
\end{verbatim}


Maybe we also want to access the true number of infected people at each time, and not just the number of students in bed. This is a latent variable for which we have an estimation.
\begin{verbatim}
params <- lapply(t, function(i){sprintf("y[%s,2]", i)}) #number of infected for each day
	smr_y <- as.data.frame(summary(fit_sir_negbin, 
	pars = params, probs = c(0.05, 0.5, 0.95))$summary)
	colnames(smr_y) <- make.names(colnames(smr_y)) # to remove % in the col names
	
	ggplot(smr_y, mapping = aes(x = t)) +
	geom_ribbon(aes(ymin = X5., ymax = X95.), fill = "orange", alpha = 0.6) +
	geom_line(mapping = aes(x = t, y = X50.)) + 
	labs(x = "Day", y = "Number of infected students")
	
\end{verbatim}


% Put complete stan program in the appendix
	
%	## Complete Stan program
%	```{stan, eval=F, output.var="md"}
%	functions {
%		real[] sir(real t, real[] y, real[] theta, 
%		real[] x_r, int[] x_i) {
%			
%			real S = y[1];
%			real I = y[2];
%			real R = y[3];
%			real N = x_i[1];
%			
%			real beta = theta[1];
%			real gamma = theta[2];
%			
%			real dS_dt = -beta * I * S / N;
%			real dI_dt =  beta * I * S / N - gamma * I;
%			real dR_dt =  gamma * I;
%			
%			return {dS_dt, dI_dt, dR_dt};
%		}
%	}
%	data {
%		int<lower=1> n_days;
%		real y0[3];
%		real t0;
%		real ts[n_days];
%		int N;
%		int cases[n_days];
%	}
%	transformed data {
%		real x_r[0];
%		int x_i[1] = { N };
%	}
%	parameters {
%		real<lower=0> gamma;
%		real<lower=0> beta;
%		real<lower=0> phi_inv;
%	}
%	transformed parameters{
%		real y[n_days, 3];
%		real phi = 1. / phi_inv;
%		{
%			real theta[2];
%			theta[1] = beta;
%			theta[2] = gamma;
%			
%			y = integrate_ode_rk45(sir, y0, t0, ts, theta, x_r, x_i);
%		}
%	}
%	model {
%		//priors
%		beta ~ normal(2, 1);
%		gamma ~ normal(0.4, 0.5);
%		phi_inv ~ exponential(5);
%		
%		//sampling distribution
%		//col(matrix x, int n) - The n-th column of matrix x. Here the number of infected people 
%		cases ~ neg_binomial_2(col(to_matrix(y), 2), phi);
%	}
%	generated quantities {
%		real R0 = beta / gamma;
%		real recovery_time = 1 / gamma;
%		real pred_cases[n_days];
%		pred_cases = neg_binomial_2_rng(col(to_matrix(y), 2), phi);
%	}
%	```





